Scalable and Efficient Temporal Graph Representation Learning via Forward Recent Sampling

Temporal graph representation learning (TGRL) is essential for modeling dynamic systems in real-world networks. However, traditional TGRL methods, despite their effectiveness, often face significant computational challenges and inference delays due to the inefficient sampling of temporal neighbors. Conventional sampling methods typically involve backtracking through the interaction history of each node. In this paper, we propose a novel TGRL framework, No-Looking-Back (NLB), which overcomes these challenges by introducing a forward recent sampling strategy. This strategy eliminates the need to backtrack through historical interactions by utilizing a GPU-executable, size-constrained hash table for each node. The hash table records a down-sampled set of recent interactions, enabling rapid query responses with minimal inference latency. The maintenance of this hash table is highly efficient, operating with $O(1)$ complexity. Fully compatible with GPU processing, NLB maximizes programmability, parallelism, and power efficiency. Empirical evaluations demonstrate that NLB not only matches or surpasses state-of-the-art methods in accuracy for tasks like link prediction and node classification across six real-world datasets but also achieves 1.32-4.40x faster training, 1.2-7.94x greater energy efficiency, and 1.63-12.95x lower inference latency compared to competitive baselines. The link to the code: https://github.com/Graph-COM/NLB.

==> 03-methodology_draft0.tex <==
%\vspace{-2mm}
\section{Methodology}\label{sec:method}





%\vspace{-1mm}
In this section, we introduce the framework of \proj. \pan{The crucial thing for this section is from top to bottom. First introduce the big several blocks before going into the details. Introduce why in the algorithmic level \proj is good. And then why in the }
On high-level \proj consists of three major components: the neighborhood cache, the motif features constructor, and the graph attention network. The neighborhood cache stores encoded history between node pairs. For each incoming event $(u, v, e, t)$, \proj reads the representations associated with $u$ and $v$ from the neighborhood cache. It then extracts the motif features according to the history of their surroundings and aggregates the motif-aware messages with a graph attention network to output the final predictions. Lastly, it updates the neighborhood cache for $u$ and $v$ based on this latest event.

These modules are very effective for the model performance. However, due to the extra memory and computation complexity, the model has to be fully optimized for real-world applications, including shrinking the memory consumption, simplifying computations, and parallelizing. We will study specific examples such as the GPU hashing algorithm which maximizes parallelism of a mini-batch with well-contained GPU memory and efficient GPU operations that work with sparse tensors.

%  We also provide a generic framework that is flexible to balance efficiency and performance as preferred for the downstream applications. Finally, it is extendable for further improvements for both efficiency and performance. For example, dynamic allocations of the neighborhood buffer for memory efficiency and the cache eviction algorithms to smartly discard old neighbors in favor of the new neighbors for higher quality neighborhood representation. 



\subsection{Neighborhood cache} \pan{at least 1 page}
The neighborhood cache is a fixed-size memory module in the GPU that is aimed to resolve the over-squashing issue. It is optimized for quick access and update to ensure model efficiency. We will first discuss our motivations. Then, we will explain the high level concepts of the neighborhood cache and dive deep into the efficiency considerations.


\subsubsection{Toward more expressive neighborhood representations}

Motivated by over-squashing. Why Message passing are insufficient. Why TGNs are insufficient. It motivated us to design the neighborhood cache. 

Motivated by CAWs, it can also used for extracting the motif features.

First, it keeps track of the identities of nodes' neighbors. They can be used for constructing the temporal network motifs~\cite{paranjape2017motifs}. CAW~\cite{wang2020inductive}'s outstanding performance on temporal link predictions empirically testifies that temporal motifs features are very effective. See section \ref{sec:motif} for more details regarding temporal network motifs in \proj.

Second, it stores the intermediate representations of a node and its neighborhood \pan{Not clear about this}. This idea stems from the memory module in TGN and the embedding trajectories in JODIE. Keeping neighborhood embeddings can effectively improve model efficiency so that they are faster than general message passing T-GNNs such as CAW~\cite{wang2020inductive} and TGAT~\cite{xu2020inductive}. The major computation bottleneck with message passing is they usually have to \begin {enumerate*}
\item look through the events associated with a node in the history (from latest to earliest), \item sample temporal edges, and \item aggregate the neighborhood states on the fly. \pan{The explanation clear is too much on efficiency but not enough for modeling needs.}
\end {enumerate*}

Third, we adopt a set of vectors for representing a node's local neighborhood. We reserve multiple representations for each node such that there is a vector dedicated to encoding the history between an origin node and another node in its neighborhood. There are two implications with this design. (1), it relieves the information bottleneck and avoids the over-squashing phenomenon. It is well-studied in \cite{alon2021on} that general GNNs suffer from over-squashing because all interactions within a node's neighborhood are compressed into a fixed-size vector. This issue is discovered recently and there is no solution for it yet. It might be natural to think that increasing the hidden size can reduce over-squashing but \cite{alon2021on} empirically showed that dimensionality increase is ineffective in preventing over-squashing. Instead, it shows that by adding a fully-adjacent layer in which every pair of nodes is connected by an edge, it achieves 42\% improvement \pan{improvement on what?} without adding weights. However, it is unrealistic and computationally expensive to assume that all node pairs are connected. Our vectors are more compact representations that replace this layer. (2), it allows information flow beyond direct neighbors without history backtracking, sampling, or stacking message passing layers. Although TGN avoids these steps with the memory module, it is unaware of messages beyond direct neighbors. To get information from the second-hop neighbors, it inevitably needs to do the backtracking and sampling. Therefore, we observe a massive slowdown in the two-layer TGN. Our neighborhood cache can represent messages from not only direct neighbors but also sub-neighborhood beyond the first hop.

\subsubsection{The neighborhood cache design}

neighborhood cache high level concept
neighborhood state definitions
neighborhood state update of when a new link comes in.
Not storing all edges or timestamp so use RNNs to get a summary.

It keeps track of the encoded states of a node and its neighborhood up to the current timestamp. A distinctive characteristic of this neighborhood cache that sets it apart from the memory modules in the existing methods like TGN \cite{tgn_icml_grl2020} is that it maintains a set of vectors for its neighborhood states instead of just a single compressed representation. The neighborhood cache is designed with three aspects.

\textbf{neighbor states}
% Each vector in the set of the neighborhood cache can be seen as a neighbor state which is dedicated to representing the interactions between a source node and each of its neighbors. Note that the interactions can be indirect in the case of multiple-hop neighbors.
For node $u \in \mathcal{V}$, suppose at the current time, it has formed a neighborhood with a set of nodes $\mathcal{N}(u) \subset \mathcal{V}$. Neighborhood cache for $u$ keeps track of a subset of $u$'s temporal neighbors, \textit{i.e.} $\mathcal{S}(u) \subset \mathcal{N}(u)$ and the timestamps of their interactions $\mathcal{T}(u)$. We also keep a collection of vectors and assign one vector for each of the neighbors we are keeping in $\mathcal{S}(u)$, \textit{i.e.} $\mathcal{C}(u) = \{c_{u,v} | v \in \mathcal{S}(u)\}$. Each vector represents a neighbor state. We encode the history between $u$ and $v$ including the link features and the temporal features into the neighbor state $c_{u,v}$ with RNNs. 
\begin{align}\label{eq:rnn}
    c_{u,v} = \text{RNN}(\{e_i \oplus F(t_i)\}_{i=0}^m) \text{ where } e_i \in \mathbb{R}^d
\end{align}
For $F(t)$, we leverage the random Fourier temporal features (Eq.\eqref{eq:randomf})to encode time. Since each neighbor state encodes a relationship between a node and its neighbor, a combination of neighbor states can represent the surroundings of a node more expressively.
% $c_{u,v} = e_{u,v} \oplus m_{u,v} \text{ where } \{e_{u,v}, m_{u,v}\} \in \mathbb{R}^d$. We encode the edge features along the previous interactions between $u$ and $v$ into $e_{u,v}$, while $m_{u,v}$ aggregates the temporal information extracted from the timestamps of those interactions. Altogether, $c_{u,v}$ represents the state of the history . 
% for the shortest paths between the source node to other nodes as shown in Fig.\ref{fig:n-cache}.To get the representation of nodes and edges in the local neighborhood without squashing,  To control the size of the neighborhood we want to consider, we limit the shortest paths to have lengths less than $k$, where $k$ is a hyper-parameter deciding within how many hops from a node we explore.
%For $f_2(t)$, we adopt random Fourier features to encode time~\citep{xu2019self,kazemi2019time2vec} which may approach any positive definite kernels according to the Bochner’s theorem~\citep{bochner1992theorem}. 

\textbf{second-hop neighbors}
Similar to the first-hop neighbors, second hop neighbors are updated when a new event $(u,v, e, t)$ comes in. We can directly sample the first-hop neighbors of $v$ to update the second hop states of $u$. The only caveat of this module is that the update is not real-time. $u$ is not aware of $v$'s new neighbors after they interacted until their next interaction. However, in practice, this asynchronous update can already provide meaningful performance gain. \yuhong{provide number x\%}


\pan{Efficient neighborhood cache update}
These expanded neighborhood states show potential in improving not only efficiency but also model expressivity. However, there are two fundamental challenges regarding their scalability. First, allocating one vector for each pair of nodes that interacted in the past consumes considerable memory. It is even more burdensome if the model needs to store extra representations for the second-hop neighbors. It does not scale for large networks with limited memory. 
%For example, the wiki-talk temporal dataset has more than 7 million static edges.
Second, throughout the learning process, we need to access and update this chunk of memory for all nodes in a mini-batch. It can easily become the computation bottleneck. To address these challenges, we introduce the GPU hashing algorithm for quick neighborhood cache operations. \pan{I do not think the explanation on how a node comes in and update the neighbors. So the motivation of GPU hashing is missing and unclear.}

fix size
Sampling
hashing
update in a batch
We first expose a hyperparameter $s$ to control the maximum number of unique neighbors allowed to be stored for each node such that the size of the cache can be maintained. Keeping a subset of total neighbors is similar to the sampling for GNNs' message passing. It is also sufficient for temporal motif feature construction \pan{This sentense you should introduce later when define what is motif features}. When CAW~\cite{wang2020inductive} extract network motifs, it samples temporal random walks and still achieves high performance. Our subsets of neighbors are precomputed asynchronously \pan{What do you mean by this?}, while other models need to sample edges from the history or the adjacency matrices during the learning. Even though there are some limitations which we will discuss in section \ref{sec:limit}, the neighborhood cache can work as an efficient replacement for other sampling methods. \pan{I do not think motif features are well defined.}

Now that the memory complexity of the cache is limited, we need to optimize the data structure to reduce the time complexity. It is natural to think of an origin node as the key and the set of neighbors as the value. In general, a hash map is the most efficient data structure for storing key-value pairs like these because accessing or updating a value to any key guarantees O(1) time complexity. Given that the adjacency matrices of most graphs are sparse, the variable-length sets are also suitable for storing node neighbors. However, this complex data structure does not easily fit into the GPU and thus is not optimized for parallelism.



\textbf{GPU Hashing}. We decided to design the data structure within GPU to allow parallel operations for all nodes in a mini-batch. Specifically, we allocate $|\mathcal{V}| \cdot s$ vectors in the GPU and initialize them with zeros. We store the neighbor states of a node $u$ into these vectors consecutively, so the $\{u \times s + j\}^s_{j=0}$ vectors belong to $u$'s neighborhood.
\textbf{Access}. 
To get the neighbor states associated with a node, we simply do an index read in the tensors. Since it does not guarantee that all preallocated slots are filled up with neighbors, we filter out empty vectors to reduce unnecessary computations with them. This will require downstream of the pipelines to work with unaligned tensors and we discuss some implementations for sparse tensors further in section \ref{sec:sparse}.
 \textbf{Update}
Suppose a new event with $u$ and $v$ arrives at time $t$ and we try to update the cache of $u$. We will first apply a hash function $0 <= f(v) \mod s$ to decide which position we store the representation of $c_{u,v}$ at. If the slot selected is empty or is already taken by $v$, we will simply update it with the hidden state of RNN of eq.~\ref{eq:rnn}. Otherwise, there is a hash collision with a previous link of $u$. Whether $v$ can occupy this slot is decided by a Bernoulli random variable with probability $p$.  Since more recent links are generally more informative, as shown in previous papers such as \cite{wang2020inductive}, we favor new links over old links. Thus, $p$ is a function that involves the time difference between the old link and the current link. It is proportional to $exp(\alpha, t_i - t)$ where $\alpha$ is a hyperparameter, such that older links are more likely to be evicted. These if-else conditions can be implemented by flipping the bits of a boolean tensor. When there are multiple events associated with the same node, it will store only one update nondeterministically. See alg \ref{alg:update}
Both the access and the update operations are all done within the GPU so can be parallelized for a mini-batch of events.
\begin{algorithm}
        \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
        $\textbf{h} \leftarrow hash(\textbf{v}) \mod s$ \;
        $\textbf{h} \leftarrow \textbf{h} + s \cdot \textbf{u} $\;
        $\textbf{o} \leftarrow \:\textcircled{$\neg$}\:((\mathcal{S}(\textbf{u})[\textbf{h}] \:\textcircled{$=$}\: \vec{\textbf{0}}) \:\textcircled{$\lor$}\: (\mathcal{S}(\textbf{u})[\textbf{h}] \:\textcircled{$=$}\: \textbf{v}))$\;
        $\textbf{r} \leftarrow [(d_i \sim U[0,1]) > exp(\alpha, T(\textbf{u})[i] - t)]_{i=0}^\text{batch size}$\;
        $\textbf{r} \leftarrow \:\textcircled{$\neg$}\:(\textbf{o} \:\textcircled{$\wedge$}\: \textbf{r}) $\;
        $\mathcal{S}(\textbf{u})[\textbf{h}] \leftarrow \textbf{v} \odot \textbf{r}$\;
        $\mathcal{C}(\textbf{u})[\textbf{h}] \leftarrow \textbf{c}$\;
        $\mathcal{T}(\textbf{u})[\textbf{h}] \leftarrow t$\;
        \caption{\small{Neighborhood Cache Batch Update ($\textbf{u}$, $\textbf{v}$, $t$, $\mathcal{C}(\textbf{u})$, $\mathcal{S}(\textbf{u})$, $\mathcal{T}(\textbf{u})$, $\alpha$, $\textbf{c}$)
        \newline Note: $hash$, \textcircled{$\neg$}, \textcircled{$=$}, \textcircled{$\wedge$}, \textcircled{$\lor$}, $\odot$ are pointwise operations }}\label{alg:update}
        \end{algorithm}
        



\subsection{Relative temporal motifs}\label{sec:motif} \pan{at least 0.5 page}

\subsubsection{The effective temporal motif features}
CAW shows that motif features are effective for distinguishing isomorphic nodes.
However, sampling is especially slow, so we leverage the neigbhorhood cache.

cross join
how to explain this?
\subsubsection{Relative motif extraction}
relative node identity.
anonymization.


\subsection{sparse implementation}\label{sec:sparse}  \pan{ One paragraph}

get from neighborhood cache

relative temporal aggregation

GAT layer with scattered

\subsubsection{sparse message passing}
\subsubsection{sparse GATs}
\subsubsection{sparse neighborhood store updates}


\subsection{Complexity analysis}

\subsection{limitations and discussions}\label{sec:limit}
3 hops. variable length neighbor. more strategic eviction.
\subsection{\yuhong{Questions}}
what should we aggregate what should not?

The motifs I can get are not exactly temporal network motifs because they are not aware of the ordering of the links. Does it matter?

Can 2nd hop hidden state of a node use the 1st hop hidden states of its direct neighbors?
Test \proj with initializing 2nd hop with default?


OGN mentions TGN also need to keep the history and sample edges. need to verify.

 There are other heuristics we can explore such as taking the number of interactions in the past in to account.

==> 03-methodology_draft1.tex <==
\section{Methodology}\label{sec:method}

In this section, we introduce the framework of \proj.
In the high level \proj consists of three major components: the neighborhood cache, the motif features constructor, and the graph attention network. The neighborhood cache stores encoded history between node pairs. For each incoming event $(u, v, e, t)$, \proj reads the representations associated with $u$ and $v$ from the neighborhood cache. It then extracts the motif features according to the history of their surroundings and aggregates the motif-aware messages with a graph attention network to output the final predictions. Lastly, it updates the neighborhood cache for $u$ and $v$ based on this latest event.

These modules are very effective for the model performance. However, due to the extra memory and computation complexity, the model has to be fully optimized for real-world applications, including shrinking the memory consumption, simplifying computations, and parallelizing for a mini-batch. We will study specific examples such as the GPU hashing and GPU inner join algorithms  which maximize parallelism of a mini-batch with well-contained GPU memory. \pan{Good}

\subsection{Neighborhood cache}\label{sec:neighborhood}
The neighborhood cache is a fixed-size memory module in the GPU that aims to resolve the over-squashing issue \pan{and structural feature construction }. It is optimized for quick access and update to ensure model efficiency. We will first discuss motivations. Then, we will explain the high level concepts of the neighborhood cache and dive deep into the efficiency considerations.


\subsubsection{Toward more expressive neighborhood representations}
The neighborhood cache is primarily motivated by the over-squashing effect of message passing. \pan{Okay, here MP does not need to review again?} Message passing (MP) is widely used for both static and dynamic graph learning~\cite{kipf2016semi, velivckovic2018graph, xu2020inductive}. It is a neural network architecture that allow messages of nodes in a graph to flow to neighboring nodes. Each node starts with a hidden representation $h$ and an MP layer aggregates hidden states of neighboring nodes to update its own representation. Each MP layer lets information flows one step in the network. By stacking multiple layers, it makes the node representation incorporate more information coming from neighbors of longer distances. While it has advantage in being aware of the structural information around the node, it introduces an information bottleneck described as the over-squashing phenomenon~\cite{alon2021on}.
\textbf{over-squashing} is well-studied in \cite{alon2021on} that general GNNs suffer from over-squashing. Since $k$-layer MP propagates information from all nodes in a $k$-hop neighborhood into a target node and squashes it into one fix-sized vector, it is going to lose some information inevitably. Over-squashing is more obvious if $k$ is larger because the number of representations it has to compress into a single vector grows exponentially with the neighborhood distance. From another perspective, representations of distanced neighbors have to go through multiple squashing before reaching the target node and the their information will be harder to generalize. As a result, over-squashing prevents GNNs from fitting the training data well, especially for nodes with rich connections.

Inspired by this novel explanation for GNNs under-fitting, we explore a way to relieve the information bottleneck \pan{Try to use another term} by avoiding squashing as much as possible. It is already shown in~\cite{alon2021on} that increasing the dimension of the destination vector is not an effective solution \pan{Interesting things}. Thus, we first increase the representation power for node neighborhood by increasing the number of vectors. Instead of representing a node, the vectors represent relationships or links between nodes. We term each vector as a \textit{relation state}. Without any quashing, a relation state can represent a part of a neighborhood on its own. A complete set of relation states associated with a node can represent the relationship between the node and its entire neighborhood. In the context of temporal network, each relation state summarizes the historical interactions between a pair of nodes.  

Formally, suppose at the current time $t$, node $u \in \mathcal{V}$, has formed a neighborhood with a set of nodes $\mathcal{N}(u) \subset \mathcal{V}$. A collection of relation states around $u$ can be represented as $\mathcal{C}(u) = \{c_{(u,v)} | v \in \mathcal{N}(u)\}$. Initialize as $c^{(0)}$ In order for $c_{(u,v)}$ to represent the relationship between $u$ and $v$, we need to leverage both the edge features and the temporal information in the history. We propose using RNNs to encode the interactions overtime. RNNs have the inductive bias of forgetting long-term memory in favor of the more recent one . It is well-suited for encoding temporal information in graphs because more recent links are generally more informative as shown in previous papers such as \cite{wang2020inductive}. We define
\begin{align}\label{eq:rnn}
    c_{u,v} = \text{RNN}(\{e_i \oplus F(t_i)\}_{i=0}^m) \text{ where } e_i \in \mathbb{R}^d
\end{align}
For $F(t)$, we leverage the random Fourier temporal features (Eq.\eqref{eq:randomf}) to encode time.
The relation states associated with a node can be used as features and fed into any pooling layer to get the final representation of the node.


\subsubsection{The introduction of neighborhood cache}
 A straight forward implementation of a model that incorporates the relation states would be as follow:\pan{I do not think it is necessary to say so much on naive implementation.}
 When the representation of a node $u$ at time $t$ is requested,
 \begin{enumerate}
     \item Sampling: sample a set of $u$'s neighbors from the adjacency matrix.
     \item Backtracking: for each $v \in \mathcal{N}_u$, look up the historical links between $u$ and $v$ to find out all interactions before $t$
     \item Encoding: for each $v \in \mathcal{N}_u$, encode the history between $u$ and $v$ with RNNs
 \end{enumerate}
 The problem with this method is that we need to repeat these steps for every training example, even for nodes we have calculated before. They become significant computation bottleneck. Thus we propose neighborhood cache for storing the intermediate results to avoid repetitive computations. It is an optimized module within the GPU that achieves O(1) parallel access and update for a mini-batch.
 
We first expose a hyperparameter $s$ to control the maximum number of unique neighbors allowed to be stored for each node such that the size of the cache can be maintained. We then allocate $s \times |\mathcal{V}|$ vectors in the GPU and initialize with zeros. We reserve $s$ vectors for each node $u \in \mathcal{V}$ for storing the relation states with neighboring nodes of $u$. The relation states for each node are stored consecutively, so the $\{u \times s + j\}^s_{j=0}$ vectors belong to $u$'s neighborhood. We denote the collection of these vectors as $\mathcal{C}$. To identify the opposite \pan{opposite?} node of the relation states, we also store a list of neighbor identities $\mathcal{S}$ in the same order as $\mathcal{C}$. The neighbor identities are also going to be used for calculating the relative temporal motifs (Sec. \ref{sec:motif}).

 \textbf{Update and eviction} We train the model with events in the order of time so that we can update the relation states as time progresses. Suppose a new event with $u$ and $v$ arrives at time $t$ and we try to update the cache of $u$. We will first apply a hash function $0 <= f(v) < s$ to decide which position we store the representation of $c_{u,v}$ at. If the slot selected is empty or is already taken by $v$, we will simply update it with the hidden state of RNNs of eq.~\ref{eq:rnn}. Otherwise, there is a hash collision with a previous neighbor $n_i \in \mathcal{N}_u$ of $u$. Whether $v$ can occupy this slot is decided by a Bernoulli random variable with probability $p$. $p$ is a function that involves the time difference between the old link and the current link. To promote new links and evict old ones, $p$ is proportional to $exp(\alpha, t_i - t)$ where $\alpha$ is a hyperparameter and $t_i$ is the timestamp of the interaction with the existing neighbor $n_i$. We store the latest timestamps of the interaction with neighbors $\mathcal{S}$ in another set $\mathcal{T}$. These if-else conditions can be implemented by flipping the bits of a Boolean tensor. When there are multiple events associated with the same node, it will store only one update nondeterministically (Alg \ref{alg:update}).

\begin{algorithm}
        \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
        $\textbf{h} \leftarrow hash(\textbf{v}) \mod s$ \;
        $\textbf{h} \leftarrow \textbf{h} + s \cdot \textbf{u} $\;
        $\textbf{o} \leftarrow \:\textcircled{$\neg$}\:[[\mathcal{S}[\textbf{h}] \:\textcircled{$=$}\: \vec{\textbf{0}}] \:\textcircled{$\lor$}\: [\mathcal{S}[\textbf{h}] \:\textcircled{$=$}\: \textbf{v}]]$\;
        $\textbf{r} \leftarrow [(d_i \sim U[0,1]) > exp(\alpha, \mathcal{T}[\textbf{h}_i] - t)]_{i=0}^\text{batch size}$\;
        $\textbf{r} \leftarrow \:\textcircled{$\neg$}\:(\textbf{o} \:\textcircled{$\wedge$}\: \textbf{r}) $\;
        $\mathcal{S}[\textbf{h}] \leftarrow \textbf{v} \odot \textbf{r}$\;
        $\mathcal{C}[\textbf{h}] \leftarrow \textbf{c}$\;
        $\mathcal{T}[\textbf{h}] \leftarrow t$\;
        \caption{\small{Neighborhood Cache Batch Update ($\textbf{u}$, $\textbf{v}$, $t$, $\mathcal{C}$, $\mathcal{S}$, $\mathcal{T}$, $\alpha$, $\textbf{c}$)
        \newline Note: $hash$, \textcircled{$\neg$}, \textcircled{$=$}, \textcircled{$\wedge$}, \textcircled{$\lor$}, $\odot$ are pointwise operations \pan{These signs are not widely used.}}}\label{alg:update}
        \end{algorithm}
    
\textbf{Access}. 
Through the training of a batch, we need to access the neighborhood cache once to get all relation states associated with a node. We simply do an index read in the tensors. Since it does not guarantee that all preallocated slots are filled up with neighbors, we filter out empty vectors to reduce unnecessary computations. Given that the number of neighbors for each node is different, it will require downstream of the pipelines to work with unaligned vectors. We discuss an efficient algorithm that smoothly operates these vectors in section \ref{sec:motif}.\pan{Here saying to postpone the intro in 4.2 is not good.}

\textbf{Beyond direct neighbors}
To avoid sampling, we also allocate a fixed-number set of vectors for each node to represent longer distance neighbors. Intuitively, this is similar to \cite{gilmer2017neural}'s virtual edges for shortening long distances and avoiding over-squashing. We use second-hop neighbors for illustration.  Similar to direct neighbors, second-hop neighbors are also updated when a new event $(u, v, e, t)$ comes in. We can directly sample the first-hop neighbors of $v$ to update the second hop states of $u$. The only caveat of this module is that the update is not real-time. $u$ is not aware of $v$'s new neighbors after they interacted until their next interaction. In practice, this asynchronous update can already provide significant performance gain. \yuhong{provide number x\%}. It also naturally captures the causality which we will explore in Sec.\ref{sec:motif}. Finally, this method can also be extended to any $k$-hop neighbors.
 



\subsection{Relative temporal motifs}\label{sec:motif} \pan{at least 0.5 page}
In order to distinguish nodes with similar local structures, we integrate the relative temporal motifs encoding between the source and the target nodes of an event into the link prediction model. This can be seen as an analogy to the distance encoding in the static GNNs~\cite{li2020distance}.
To extract the motif features, we leverage temporal walks. This is an idea inspired by CAW~\cite{wang2020inductive}. However CAW is inefficient because it samples random walks for each node by backtracking over time to extract motifs. To avoid backtracking, we leverage the neighborhood cache (Sec. \ref{sec:neighborhood}).

\subsubsection{Encoding of a powerful structural feature}
We are interested in temporal motifs because they capture both the structural patterns and the temporal information. To abstract temporal motif features, we start with temporal walks. Although temporal walks resemblance the temporal motifs, temporal walks have explicit node identities and timestamps such that they do not generalize as well as temporal motifs. An important step toward transforming temporal walks to temporal motifs is anonymization of nodes and abstraction of timestamps.

We cannot simply remove node identities from temporal walks because a walk contains structural information that is related to node identities. We propose anonymizing node identities with distance encoding (DE) \cite{li2020distance}. There are different DE variants. We will focus on the shortest path distance (SPD) because it is the simplest while it does not perform worse than other methods in practice.
The SPD of node $a$ in a set of temporal walks $S=\{W_1, W_2, ..., W_M\}$ is defined as
\begin{equation}
    \tilde{g}(a; S)\triangleq i,
    \text{where } i=\min\{j|\exists W\in S, a \text{ appears at }W[j]\}. 
    \label{eq:spd}
\end{equation} 
To abstract timestamps, we only need to keep track of the order in which the edges
occur as described in \cite{paranjape2017motifs}. Because temporal walks follow edges in the descending order of time, they naturally encode the temporal structure. Thus, we can simply drop the timestamps of temporal walks.


\subsubsection{extracting motifs from neighborhood cache}
While the most straight forward approach to obtain the temporal walks is the temporal random walk proposed in~\cite{wang2020inductive}, it requires backtracking history and sampling walks which lead to computation bottleneck. Thus, we leverage the neighborhood cache to avoid random walk sampling. Because we update and evict neighbors with randomness, and keep direct and $2^{nd}$ hop neighbors in separate caches, they naturally represent a fragmented random walk. Furthermore, thanks to our delayed update of multiple-hop neighbors, the links to the 2-nd hop neighbors usually appear earlier and therefore, they follow the temporal ordering of temporal walks. Since neighborhood cache is aware of the distances of the neighbors to the source node, we can easily arrive at the SPD of nodes in temporal walks.

\begin{figure}
\includegraphics[width=0.45\textwidth]{Relative motifs.png}
%   \vspace{-6.5mm}
%\hspace{-3mm}
\caption{\small{Left: the neighbors stored in the caches. Assume it is storing the complete neighbors. Middle: the subgraphs inferred from a single source, either A or B. Right: the sub-graphs inferred combining neighborhoods of both A and B. Note that anonymizing the node ids in the subgraphs produces the motifs. } }
\label{fig:relative} \end{figure}

We have been talking about generating motif features from a single source node. However, it is not sufficient as shown in (Fig.\ref{fig:relative}. Given neighbor ids $\textbf{s}_u$, we can infer an incomplete subgraph around $u$. However, it can miss important structural information because (1), the neighborhood is incomplete. we sample the neighbors and our update beyond first hop is delayed. (2), The neighborhood cache is not aware of the links between the neighbors.
Thus, if the opposite node $v$ happens to be one of the neighbors of $u$, we can fill in missing links and expand the neighborhood. The motifs extracted from this augmented subgraph -- termed relative motifs, are far more informative than motifs of a single source. As an example, Fig.\ref{fig:relative} demonstrates that single-source subgraphs do not capture the the link (B,C) and (C,D) while the combined subgraph does. We will empirically compare the motif features with single source v.s. the relative motifs features. CAW has also showed that the random walks from a single source is insufficient while merges random walks from both sources boosts the model performance.


Alg.~\ref{alg:motif} introduces the algorithm to extract relative motif feature from the sub-neighborhoods of source node $u$ and target $v$, i.e. $\textbf{s}_u$ and $\textbf{s}_v$ retrieved from the neighborhood cache. The vector operations can all be done within the GPU and thus can be parallelized for a mini-batch. All $\textbf{g}^{(i,j)}_u$ can be used as features to calculate $u$'s final embedding.
\begin{algorithm}
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
 \For{$i$ from $1$ to $m$, the $i-$th step}{
    $l \leftarrow \textit{one hot}(i)$\;
    $\textbf{l}^{(i)}_u \leftarrow
  \bigl[ \underbrace{%
    l \quad  l \quad  \cdots \quad  l
  }_{\text{$|\textbf{s}^{(i)}_u| $~elements}} \bigr]$\;
  $\textbf{l}^{(i)}_v \leftarrow
  \bigl[ \underbrace{%
    l \quad  l \quad  \cdots \quad  l
  }_{\text{$|\textbf{s}^{(i)}_v| $~elements}} \bigr]$\;
 }
 
 \For{$i$ from $1$ to $m$, the $i-$th step}{
    \For{$j$ from $1$ to $m$, the $j-$th step}{
        $\textbf{s}_{all} \leftarrow [\textbf{s}^{(i)}_u ||  \textbf{s}^{(j)}_v]$\;
        $\textbf{uni}, \textbf{idx} \leftarrow $ find unique elements in $\textbf{s}_{all}$; also return original indices of the unique elements\;
        $\textbf{l}_{all} \leftarrow [\textbf{l}^{(i)}_u || \textbf{l}^{(j)}_v]$\;
        $\textbf{f}^{(i,j)} \leftarrow \bigl[ \underbrace{%
    0 \quad  0 \quad  \cdots \quad  0
  }_{\text{$|\textbf{uni}| $~elements}} \bigr]$\;
        Scatter add $\textbf{l}_{all} $ to $\textbf{f}^{(i,j)}$ according to indices in $\textbf{idx}$\;
        $\textbf{g}^{(i,j)} \leftarrow \bigl[ \underbrace{%
    0 \quad  0 \quad  \cdots \quad  0
  }_{\text{$|\textbf{idx}| $~elements}} \bigr]$\;
        Assign elements in $\textbf{f}^{(i,j)} $ to $\textbf{g}^{(i,j)}$ according to indices in $\textbf{idx}$\;
        $\textbf{g}^{(i,j)}_u \leftarrow \textbf{g}^{(i,j)}[1, 2, \quad \cdots \quad , |\textbf{s}^{(i)}_u|]$\;
        $\textbf{g}^{(i,j)}_v \leftarrow \textbf{g}^{(i,j)}[|\textbf{s}^{(i)}_u|, |\textbf{s}^{(i)}_u| + 1, \quad \cdots \quad, |\textbf{s}^{(j)}_v|]$\;
    }
 }
\caption{\small{Relative motifs aggregation ($\textbf{s}_u$, $\textbf{s}_v$, $m$) }}\label{alg:motif}
\end{algorithm}

\subsection{Graph attention output layer}
We propose a simple single-layer GAT~\cite{velivckovic2018graph} to summarize the neighbors information conveyed by the relation states and the relative motif features and generate a final node representation. We layout all neighbors sampled and treat them all as the direct neighbors. Following GAT, we will first calculate the attention scores with 
\begin{align}\label{eq:attention}
    \alpha_{ij} = \frac{exp(\text{LeakyReLU}(\textbf{a}^T[\textbf{W}\textbf{h}_i||\textbf{W}\textbf{h}_j]))}
    {\sum_{k\in \mathcal{N}_i} exp(\text{LeakyReLU}(\textbf{a}^T[\textbf{W}\textbf{h}_i||\textbf{W}\textbf{h}_k]))}
\end{align}
where \textbf{a} is a learnable weight vector of a single-layer feedforward neural network, \textbf{W} is a weight matrix that project input features into higher-level features, one for each attention head.

Next, we aggregate the projected features according to the attention score and produce the final embedding. Formally, it can be expressed as:
\begin{align}\label{eq:final_sum}
    \textbf{o}_i = \sigma(\sum_{j\in \mathcal{N}_i}\alpha_{ij} \textbf{W}\textbf{h}_j)
\end{align}
where $\sigma$ is a nonlinearity activation.

Here we also leverage the scatter add method so we can parallelize all nodes in a mini-batch even though the number of neighbors are unaligned for the nodes.

==> 04-theoretical.tex <==
\setlength{\columnsep}{15pt}
\section{Theoretical Analysis [Ready for review]}\label{sec:theory}
\pan{sec 5 should be put into sec 4 with the mechanism together.}


In this section, we first defines 3 sampling strategies, recent truncation, uniform sampling and recent sampling as used by previous work \pan{recent truncation and uniform sampling should be mentioned as the prelim. And say they are not good. We then mainly discuss recent sampling and how it can be fast implemented via hash (note that we should provide ab studies on using different sampling via our backbones).}, and show that \proj-edge which uses edges, e.g., $e_{u,v}^t$ as hash key to DHT is equivalent to recent sampling. We then introduce a new sampling strategy called recent node-wise sampling which is followed by \proj-node which uses neighbor IDs, e.g., $v$ as hash keys. \pan{if node-wise sampling does not give good performance, maybe we do not need to do that.}

We first denote the list of downsampled neighbors to be aggregated for learning a node representation of $u$ at time $t$ as $\Gamma$ \pan{the notation is suggested to be consistent with the previous one, e.g., $\hat{\mathcal{N}}^t_u$} and the size is $S$ \pan{suggest to use little letter such as $s$, $m$, $n$}.
%
To characterize each of the sampling strategies, we consider the probability a temporal neighbor gets selected as one of $\Gamma$. Let $N_i \coloneqq (v_i, e^{t_i}_{u,v_i}, t_i)$ and $N_i \in \mathcal{N}^t_u$  be one of the historical temporal neighbors of $u$, where $ i \in \bigg[1, |\mathcal{N}^t_u|\bigg]$.

\pan{suggest recent truncation and uniform sampling mentioned in the prelim work. In the intro, we want to list a table of all sampling methods if it may help.}
\subsection{Recent truncation} Recent truncation is a common strategy used by TGN and TGL. It does not sample with randomness but truncates the most recent $S$ temporal neighbors that appear in the history instead. Thus, \pan{recent truncation and uniform sampling are simple, I do not think we need to write in this formal way.}
\begin{align}
\Pr(N_i \in \Gamma) = \begin{cases}
  0  & i \le |\mathcal{N}^t_u| - S, \\
  1 & \text{otherwise.}
\end{cases}
\end{align}
\textbf{Time complexity.} Suppose one performs the traditional backtracking and sampling online, its time complexity is $\mathcal{O}(S)$.

\subsection{Uniform sampling} Uniform sampling is also commonly supported by TGN, TGL, TGAT, etc. Although it is a straightforward strategy for sampling, it suffers from even larger latency because it needs to backtrack and access all of the historical temporal interactions. We formulate the probability below,
\begin{align}
\Pr(N_i \in \Gamma) = \frac{S}{|\mathcal{N}^t_u|}.
\end{align}
\textbf{Time complexity.} Suppose one performs the traditional backtracking and sampling online, its time complexity is $\mathcal{O}(S \times |\mathcal{N}^t_u|)$.

\subsection{Recent sampling}
Recent sampling is proposed by TGAT and CAWN \pan{references?}. It backtracks the historical interactions and samples with a larger weight for the more recent interactions. It has shown to be effective for some scenarios as it both leverages recency and randomness of the temporal neighbors. \pan{We should introduce why this may be very computationally costly: Introduce high latency.}

According to the sampling strategy proposed in CAWN, $\Pr(N_i \in \Gamma)$ is proportional to $\text{exp}(c(t_i - t))$ where $c > 0$ is a constant.
%Then, \pan{what is $N_j$ summed over? }
%\begin{align}
% \Pr(N_i \in \Gamma) = \frac{\text{exp}(c(t_i - t))}{\sum_{N_j} \text{exp}(c(t_j - t))}.
% \end{align}
\textbf{Time complexity.}  Suppose one performs the traditional backtracking and sampling online, its time complexity is $\mathcal{O}(S \times |\mathcal{N}^t_u|)$.

Next, we prove that \proj-edge's DHT achieves equivalent sampling mechanism under the following assumption. \pan{As this assumption is simple, we do not need to list it separately. Merge it into the statement of the theorem.}

\begin{assumption} [Edges arrive following Poisson point process.]
We assume that links come in for node $u$ by following a Poisson point process with intensity $\lambda$. It is a commonly
used assumption to model communication networks~\citet{lavenberg1983computer} and an assumption used in CAWN \pan{the second statement is typically put in the remark instead of the formal statement}.
\end{assumption}
\begin{theorem}[\proj-edge achieves recent sampling.]\label{thm:edge} \pan{where is the statement?}
\end{theorem}
\textit{Proof.}
We aim to prove that $\Pr(N_i \in \Gamma)$ is proportional to $\text{exp}(c(t_i - t))$. First, the probability that $N_i$ or any other temporal neighbors is inserted to $\Gamma$ is $\alpha$ as we define in Sec.~\ref{sec:mantenance}.

Suppose $N_i$ is inserted to $\Gamma$ \pan{here we have another $\alpha$ prob}, we then evaluate the probability that it does not get replaced by another temporal neighbor. We know from the Poisson process that there are $\lambda (t_i - t)$ \pan{$\lambda (t-t_i)$} links arrive since $t_i$ \pan{this is just in expectation, a more formal way to state this is needed}. On average, each link has probability $\frac{\alpha}{S}$ of replacing $N_i$ \pan{here, we also assume that hash is purely uniformly random. Then, do we still want to say that we are using hash? Why not just randomly insertion?}. Then the expected number of links that are inserted to the same position as $N_i$ is $\frac{\alpha\lambda}{S} (t_i - t)$ \pan{$\frac{\alpha\lambda}{S} (t-t_i)$}  and the intensity of links being inserted to the same position as $N_i$ is $\frac{\alpha\lambda}{S}$.

By the property of a Poisson process, the probability that none of the links get inserted to the same position as $N_i$ from $t_i$ to $t$ is $\text{exp} (\frac{\alpha\lambda}{S} (t_i - t))$. Overall, 
\begin{align}
    \Pr(N_i \in \Gamma) = \alpha ~ \text{exp}(\frac{\alpha\lambda}{S} (t_i - t)).
\end{align}\pan{not sure if this is correct unless giving the correct setup: This probability is that given an interaction at $t_i$,  the probability of this interaction is still kept in the DHT at time $t$. A looking-forward probability instead of a looking-backward probability as CAWN used.} 
We have shown that $\Pr(N_i \in \Gamma)$ is proportional to $\text{exp}(c(t_i - t))$ for $c > 0$, completing the proof.

\subsection{Recent node-wise sampling} \pan{if this method does not work well, we do not need to mention this in the main text. We just need to mention that we also tried this approach and it does not work well because xxx. If you want to add some results of this setting, put them in the appendix}

We propose a new recent sampling strategies that considers the probability a distinct neighbor ID being selected where temporal neighbors with the same neighbor ID are deduplicated. This strategy can speed up the aggregation of a node's neighborhood as it reduces the number of sampled candidates. Specifically, let $\mathcal{U}_u^t$ be a subset of $\mathcal{N}_u^t$ that records the last appearance of every static neighbor $v_i$. Let $U_i \coloneqq (v_i, e^{t_i}_{u,v_i}, t_i) \in \mathcal{U}_u^t$.

We require the recent node-wise sampling to satisfy $\Pr(U_i \in \Gamma) \propto b + \text{exp}(c(t_i - t))$ where both $b > 0$ and $c>0$ are constant.

We now prove that \proj-node achieves recent node-wise sampling under the following assumption.

\begin{assumption} [Different static neighbors follow different independent Poisson processes.]
We assume that links to neighbor $v_i$ come in for node $u$ by following a Poisson point process with intensity $\lambda_{v_i}$ and each neighbor follows a different and independent process to other neighbors.
\end{assumption}
\begin{theorem}[\proj-node achieves recent node-wise sampling.]
\end{theorem}
\textit{Proof.}
\proj-node
%only consider unique node IDs with the most recent edge features and timestamps. 
hashes by node ID. Thus, the probability a different neighbor $v_j$ hashes to the same position as $v_i$ is $\frac{1}{S}$. Similar to the argument in Theorem~\ref{thm:edge}, for $v_j$, during $(t_i, t)$, there are $\alpha\lambda_{v_j}$ temporal neighbors associated with neighbor $v_j$ gets inserted into $\Gamma$.  The probability none of the links associated with a neighbor $v_j$ is inserted during $(t_i, t)$ is then $\text{exp}(\alpha\lambda_{v_j}(t_i - t))$, according to the property of a Poisson process.

For the event $U_i\in \Gamma$ to happen, it has to be true that for all neighbors $v_j$ that $v_j \ne v_i$, $\text{hash}(v_j) \ne \text{hash}(v_i)$  or none of the links associated with a neighbor $v_j$ is inserted to $\Gamma$ during $(t_i, t)$. Overall, 
\begin{align}
    \Pr(U_i \in \Gamma) &= \alpha ~ \bigg(\frac{S-1}{S} + \frac{1}{S} \prod_{v_j\in~ \mathcal{U}_u^t \setminus \{v_i\} } \text{exp}(\alpha\lambda_{v_j} (t_i - t))\bigg)\\
    &= \alpha ~ \bigg(\frac{S-1}{S} + \frac{1}{S} \text{exp}(\alpha\sum_{v_j\in ~\mathcal{U}_u^t\setminus \{v_i\} } \lambda_{v_j}(t_i - t))\bigg)
\end{align}

Thus, $\Pr(U_i \in \Gamma) \propto b + \text{exp}(c(t_i-t))$ with $b > 0$ and $c > 0$, completing the proof. \textcolor{red}{This proof assumes $H_u^t[\text{hash}(v_i)]$ is non-empty before $U_i$  arrives.}
% \subsection{Assumption.} For each node $u$, we suppose neighbors $\mathcal{N}_u^t$ follows a Poisson process. Mathematically,  Suppose $v$ is one of $u$'s neighbors. We denote the rate of the Poisson process for neighbor $v$ as $\lambda_v$.

% Suppose neighbors $1\ldots G$ hash to the same position $\rho$ as neighbor $v$ in the N-cache of $u$. We prove that at timestamp $T$, whether the N-cache at $\rho$ keeps $v$ follows a probability distribution with parameters $\lambda_1\ldots \lambda_G, \lambda_v$. 

% $$P(\mathcal{N}_u^T[\rho] = v) = \int_0^T (1 - \lambda_v * e^{(-\lambda_v * t)}) * \alpha * \prod_{g=1}^G \left(1 - (1 - \lambda_g * e^{(-\lambda_g * t)}) * \alpha \right)\,dt$$.

% When a link with neighbor $g$ arrives, we insert $g$ into the N-cache with probability $\alpha$.
% Suppose N-cache at $\rho$ is current not $g$. Then the probability N-cache at $\rho$ gets neighbor $g$ within the next time interval of length $t$ is,\\
% $P(g $ inserted during interval $ t) = P(g $ arrives during interval $ t) * \alpha = (1 - \lambda_g * e^{(-\lambda_g * t)}) * \alpha$.
% Then $P(g $ not inserted during interval $ t) = 1 - (1 - \lambda_g * e^{(-\lambda_g * t)}) * \alpha$.

% The probability $P(\mathcal{N}_u^T[\rho] = v)$ is the probability when the latest neighbor get inserted into $\rho$ is exactly $v$. Equivalently, if after an arbitrary time $t < T$, $v$ is inserted while all other neighbors with the same hash are not inserted, it is guaranteed that $\mathcal{N}_u^T[\rho] = v$. Then \begin{align}
%     & P(\mathcal{N}_u^T[\rho] = v) \\ &=\int_0^T P(v \text{ inserted during interval } (T-t)) * \prod_{g=1}^G P(g \text{ not inserted during interval } (T-t)) \,dt\\
%     &=\int_0^T P(v \text{ inserted during interval } t) * \prod_{g=1}^G P(g \text{ not inserted during interval } t) \,dt\\
%     &=\int_0^T (1 - \lambda_v * e^{(-\lambda_v * t)}) * \alpha * \prod_{g=1}^G \left(1 - (1 - \lambda_g * e^{(-\lambda_g * t)}) * \alpha \right)\,dt
% \end{align} 

